Untangling Carbon-free Energy Attribution and Carbon Intensity Estimation for Carbon-aware Computing

Many organizations, including governments, utilities, and businesses, have set ambitious targets to reduce carbon emissions for their Environmental, Social, and Governance (ESG) goals. To achieve these targets, these organizations increasingly use power purchase agreements (PPAs) to obtain renewable energy credits, which they use to compensate for the ``brown'' energy consumed from the grid. However, the details of these PPAs are often private and not shared with important stakeholders, such as grid operators and carbon information services, who monitor and report the grid's carbon emissions. This often results in incorrect carbon accounting, where the same renewable energy production could be factored into grid carbon emission reports and separately claimed by organizations that own PPAs. Such ``double counting'' of renewable energy production could lead organizations with PPAs to understate their carbon emissions and overstate their progress toward sustainability goals, and also provide significant challenges to consumers using common carbon reduction measures to decrease their carbon footprint. Unfortunately, there is no consensus on accurately computing the grid's carbon intensity by properly accounting for PPAs. The goal of our work is to shed quantitative and qualitative light on the renewable energy attribution and the incorrect carbon intensity estimation problems.

==> 7-discussions-future-work.tex <==
If everyone follows only location- or market-based carbon accounting, there is no double counting~\cite{holzapfel2023electricity}, and the toy examples for double counting and reporting discrepancy we have shown in this paper will not apply. However, following only location-based carbon accounting is unlikely, given the increasing trend of buying PPAs and the push towards 24/7 carbon-free energy. For market-based accounting, there is currently a need for both data availability and new algorithms to handle all the nuances. Currently, residual grid data is only available annually and lags for a few years~\cite{aib_residual, green_e_residual}. Data about PPAs, the amount of renewables removed from the grid due to such PPAs, and the residual grid mix are needed at an hourly scale if we are to move towards true decarbonization. Efforts are required from both the buyers and sellers of PPAs to make such data available in real-time and increase the visibility of the electrical grids and electricity markets. 

Even if data is available, there are other challenges since electricity consumed in a region is often a mix of locally produced and electricity imported from the nearby regional grids. The current consumption-based algorithms~\cite{de2019tracking, tranberg2019real, horsch2018flow, tranberg2015power, bialek1996tracing, abdelkader2007transmission, kirschen1999tracing, schafer2019principal, li2013carbon} are not well equipped to capture the effect of PPAs on the total and residual grid mix of a region, and this situation becomes more complex when electricity is imported from another region which itself has PPAs. Although there have been recent efforts in calculating the residual grid mix~\cite{kuronen2020issue, residual_mix_calc_2020}, developing new algorithms to calculate the consumption-based CI at an hourly scale while considering PPAs is an essential future direction and one that needs our urgent attention. Once data is available, a hierarchical algorithm that calculates the residual mix by removing the renewables and then applying one of the existing techniques may be a reasonable first step towards accurate carbon-free energy attribution and correct emission reporting.
Only when both the data and PPA-aware algorithms are available will current carbon-aware optimizations be able to truly reduce the carbon emissions associated with electricity consumption and lead towards a greener future.

